ILLUME+: Illuminating Unified MLLM with Dual Visual Tokenization and Diffusion Refinement

We present ILLUME+ that leverages dual visual tokenization and a diffusion decoder to improve both deep semantic understanding and high-fidelity image generation. Existing unified models have struggled to simultaneously handle the three fundamental capabilities in a unified model: understanding, generation, and editing. Models like Chameleon and EMU3 utilize VQGAN for image discretization, due to the lack of deep semantic interaction, they lag behind specialist models like LLaVA in visual understanding tasks. To mitigate this, LaViT and ILLUME employ semantic encoders for tokenization, but they struggle with image editing due to poor texture preservation. Meanwhile, Janus series decouples the input and output image representation, limiting their abilities to seamlessly handle interleaved image-text understanding and generation. In contrast, ILLUME+ introduces a unified dual visual tokenizer, DualViTok, which preserves both fine-grained textures and text-aligned semantics while enabling a coarse-to-fine image representation strategy for multimodal understanding and generation. Additionally, we employ a diffusion model as the image detokenizer for enhanced generation quality and efficient super-resolution. ILLUME+ follows a continuous-input, discrete-output scheme within the unified MLLM and adopts a progressive training procedure that supports dynamic resolution across the vision tokenizer, MLLM, and diffusion decoder. This design allows for flexible and efficient context-aware image editing and generation across diverse tasks. ILLUME+ (3B) exhibits competitive performance against existing unified MLLMs and specialized models across multimodal understanding, generation, and editing benchmarks. With its strong performance, ILLUME+ provides a scalable and versatile foundation for future multimodal applications. Project Page: https://illume-unified-mllm.github.io/.

==> tables/method_data_composition.tex <==
\begin{table}[t]
\centering
\tablestyle{2.5pt}{1}
\begin{tabular}{lll}
\hline
Type                                      & Dataset                                         & \# Samples \\ \hline
\multirow{5}{*}{Multimodal Understanding} & Private Dataset                                 & 10M        \\
                                          & EMOVA Pretrain \cite{chen2024emova}             & 3.1M       \\
                                          & EMOVA SFT \cite{chen2024emova}                  & 3.8M       \\
                                          & Pixmo \cite{deitke2024molmo}                    & 262K       \\
                                          & M4-Instruct \cite{liu2024improved}              & 100K       \\ \hline
Image Reconstruction                      & Wukong100M \cite{gu2022wukong}                                 & 6M         \\ \hline
\multirow{2}{*}{Text-to-image Generation} & In-house Aesthetic Dataset                      & 37M        \\
                                          & COYO \cite{kakaobrain2022coyo-700m}             & 3M         \\ \hline
\multirow{6}{*}{Image Editing}            & Private Dataset                                 & 532K       \\
                                          & UltraEdit \cite{zhao2024ultraedit}              & 1.2M       \\
                                          & SEED-Edit \cite{ge2024seed}                     & 16K        \\
                                          & AnyEdit \cite{yu2024anyedit}                    & 1.8M       \\
                                          & OmniEdit \cite{wei2024omniedit}                 & 1.2M       \\
                                          & Instruct-Pix2Pix \cite{brooks2023instructpix2pix}          & 50K        \\ \hline
\multirow{5}{*}{Text-to-Text}             & Magpie Datasets \cite{xu2024magpie}           & 1.7M       \\
                                          & OpenOcra \cite{OpenOrca}                  & 4.2M       \\
                                          & OpenHermes \cite{OpenHermes2.5}                & 243K       \\
                                          & OPC-SFT-Stage1 \cite{Huang2024OpenCoderTO}             & 1.5M       \\
                                          & SCP-116K \cite{lu2025scp}                  & 43K        \\ \hline
\end{tabular}
\caption{Details of dataset composition.}
\label{tab:data_composition}
\end{table}

==> tables/result_additional_generation.tex <==
\begin{table}[ht]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \scriptsize
    \vspace{-2mm}
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Method} & \textbf{Global} & \textbf{Entity} & \textbf{Attribute} & \textbf{Relation} & \textbf{Other} & \textbf{Overall$\uparrow$} \\
        \midrule
        \multicolumn{7}{c}{\it Generation-specific Models.} \\
        \midrule
        SDv1.5 \cite{rombach2022high} & 74.63 & 74.23 & 75.39 & 73.49 & 67.81 & 63.18 \\
        PixArt-$\alpha$ \cite{chen2023pixart} & 74.97 & 79.32 & 78.60 & 82.57 & 76.96 & 71.11 \\
        Lumina-Next~\cite{liu2024lumina} & 82.82 & 88.65 & 86.44 & 80.53 & 81.82 & 74.63 \\
        SDXL~\cite{podell2023sdxl} & 83.27 & 82.43 & 80.91 & 86.76 & 80.41 & 74.65 \\
        Playground v2.5~\cite{mjhq} & 83.06 & 82.59 & 81.20 & 84.08 & 83.50 & 75.47 \\
        Hunyuan-DiT~\cite{li2024hunyuan} & 84.59 & 80.59 & 88.01 & 74.36 & 86.41 & 78.87 \\
        PixArt-$\Sigma$~\cite{chen2024pixart_sigma} & 86.89 & 82.89 & 88.94 & 86.59 & 87.68 & 80.54\\
        Emu3-Gen~\cite{wang2024emu3} & 85.21 & 86.68 & 86.84 & 90.22 & 83.15 & 80.60 \\
        DALL-E 3~\cite{betker2023improving} & 90.97 & 89.61 & 88.39 & 90.58 & 89.83 & 83.50 \\
        SD3-Medium \cite{stable_diffusion_3} & 87.90 & 91.01 & 88.83 & 80.70 & 88.68 & 84.08 \\
        \midrule
        \multicolumn{7}{c}{\it Unified Understanding and Generation Models} \\
        \midrule
        Janus~\cite{wu2024janus} & 82.33 & 87.38 & 87.70 & 85.46 & 86.41 & 79.68 \\
        Janus-Pro-1B~\cite{chen2025janus_pro} & 87.58 & 88.63 & 88.17 & 88.98 & 88.30 & 82.63 \\
        Janus-Pro-7B~\cite{chen2025janus_pro} & 86.90 & 88.90 & 89.40 & 89.32 & 89.48 & 84.19 \\

        ILLUME~\cite{wang2024illume} & \\
        \textbf{\method-3B} & 84.5 & 83.7 & 85.91 & 89.86 & 86.52 & 79.6 \\
        \bottomrule
    \end{tabular}
    %}
    \caption{Performances on DPG-Bench.}
    \label{tab:exp-dpg}
    \vspace{-4mm}
\end{table}


==> tables/result_editing.tex <==
\begin{table}[h]
\center
\setlength{\tabcolsep}{3.6pt}
\Large
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcc|cccc}
\toprule
 & & & \multicolumn{4}{c}{\it Emu Edit}  \\
\multirow{-2}[0]{*}{Method} & \multirow{-2}[0]{*}{Type} & \multirow{-2}[0]{*}{Tasks} & DINO & CLIP-I & CLIP-T & CLIP-DIR \\
\midrule
InstructPix2Pix~\cite{brooks2023instructpix2pix} & Diffusion & Edit only & 0.762 & 0.834 & 0.219 & 0.078 \\
MagicBrush~\cite{zhang2024magicbrush} & Diffusion & Edit only & 0.776 & 0.838 & 0.222 & 0.09\\
OmniGen~\cite{xiao2024omnigen} & Diffusion & Edit only & 0.804 & 0.836 & 0.233 & -\\
Emu Edit~\cite{emuedit} & Diffusion & Edit only & \underline{0.819} & 0.859 & 0.231 & \textbf{0.109}\\
\midrule
PUMA~\cite{fang2024puma} & AR & Edit only & 0.785 & 0.846 & \underline{0.270} & -\\
ILLUME & AR & Und, Gen, Edit & 0.791 & \textbf{0.879} & 0.260 & - \\
\rowcolor{backgroundcolor} \method~ & AR & Und, Gen, Edit & \textbf{0.826} & \underline{0.872} & \textbf{0.275} & \underline{0.101} \\
\bottomrule
\end{tabular}
}
% \vspace{-2mm}
\caption{\textbf{Quantitative results on image editing benchmarks. } The performance with top-1 and top-2 value are denoted in bold and underline respectively.%AR denotes autoregressive.
}
% \vspace{-4mm}
\label{tab:editing_results}
\end{table}
